Efficient and realistic 3-D Boundary Element simulations of underground construction using isogeometric analysis

The paper outlines some recent developments of the boundary element method (BEM) that makes it more user friendly and suitable for a realistic simulation in geomechanics, especially for underground excavations and tunnelling. The innovations refer to the introduction of isogeometric concepts, elasto-plastic analysis and the simulation of ground support. The introduction of isogeometric concepts for the description of the excavation boundaries results in less user and analysis effort, since complex geometries can be modelled with few parameters and degrees of freedom. No mesh generation is necessary. In order to consider heterogeneous and inelastic ground conditions a domain discretisation is used but the use of isogeometric methods results in a minimum of user effort. Efficient methods are also presented for modelling rock bolts. A comparison of results of test examples with other numerical methods and analytical solutions confirm the efficiency and accuracy of the proposed implementation. A practical example with a complex geometry is presented.

==> settings/myheadings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % myheadings.tex
% %
% % 	requires:		\usepackage{scrpage2}
% % 				\usepackage{setspace}
% %

%%% Headings
%\pagestyle{headings}
\automark[chapter]{section}
\pagestyle{scrheadings}
% \rehead{\chaptermark}
\chead{}
\rohead[]{\pagemark}
%\rohead{\pagemark}
%\lohead{\rightmark}
\lohead{\rightmark}
\rehead{\leftmark}
% \lehead{}
\lehead{\pagemark}
\lefoot{}
\cefoot[]{}
\cofoot[]{}
% \rofoot[\pagemark]{\pagemark}
\rofoot[]{}
\setheadsepline{1pt}

%%% Vertical offset of chapters (standard is 1.8)
\renewcommand*{\chapterheadstartvskip}{\vspace{2.2\baselineskip}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 

